Parallelized Rate-Distortion Optimized Quantization Using Deep Learning

Rate-Distortion Optimized Quantization (RDOQ) has played an important role in the coding performance of recent video compression standards such as H.264/AVC, H.265/HEVC, VP9 and AV1. This scheme yields significant reductions in bit-rate at the expense of relatively small increases in distortion. Typically, RDOQ algorithms are prohibitively expensive to implement on real-time hardware encoders due to their sequential nature and their need to frequently obtain entropy coding costs. This work addresses this limitation using a neural network-based approach, which learns to trade-off rate and distortion during offline supervised training. As these networks are based solely on standard arithmetic operations that can be executed on existing neural network hardware, no additional area-on-chip needs to be reserved for dedicated RDOQ circuitry. We train two classes of neural networks, a fully-convolutional network and an auto-regressive network, and evaluate each as a post-quantization step designed to refine cheap quantization schemes such as scalar quantization (SQ). Both network architectures are designed to have a low computational overhead. After training they are integrated into the HM 16.20 implementation of HEVC, and their video coding performance is evaluated on a subset of the H.266/VVC SDR common test sequences. Comparisons are made to RDOQ and SQ implementations in HM 16.20. Our method achieves 1.64% BD-rate savings on luminosity compared to the HM SQ anchor, and on average reaches 45% of the performance of the iterative HM RDOQ algorithm.

==> data/ebu_dataset.tex <==
%\begin{table}[t!]
%\caption{\hl{REMOVE} The sampled number of blocks from the \ebu dataset, in millions, for training (top rows) and validation (bottom rows) for the different prediction structures and quantization parameters. 
%Dana, please update this table with AI 37 blocks if possible!
%}
%\label{tab:ctc}
%
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{lrrr|rrr|rrr}
%\toprule
% {} &     \multicolumn{3}{c}{AI} &  \multicolumn{3}{c}{RA}  & \multicolumn{3}{c}{LPP}  \\
% {} &     \multicolumn{1}{c}{22} & \multicolumn{1}{c}{27} & \multicolumn{1}{c}{32} & \multicolumn{1}{c}{22} & \multicolumn{1}{c}{27} & \multicolumn{1}{c}{32} & \multicolumn{1}{c}{22} & \multicolumn{1}{c}{27} & \multicolumn{1}{c}{32} \\
%\midrule
%RainFruits  &   2.91 &   1.87 &   1.25 &   1.43 &   0.56 &   0.28 &     2.77 &     1.17 &     0.59 \\
%LupoCandlelight &   3.95 &   1.45 &   0.72 &   1.86 &   0.42 &   0.16 &     3.52 &     0.57 &     0.22 \\
%WindWool    &   3.83 &   2.29 &   1.55 &   1.96 &   0.88 &   0.49 &     2.83 &     1.25 &     0.67 \\
%VeggieFruits &   3.30 &   1.94 &   1.17 &   1.29 &   0.49 &   0.23 &     2.39 &     0.89 &     0.40 \\
%PendulusWide &   5.07 &   2.81 &   1.95 &   2.83 &   1.01 &   0.54 &     5.23 &     1.82 &     0.98 \\
%LupoBoa     &   3.82 &   1.37 &   0.78 &   3.63 &   2.10 &   1.26 &     4.31 &     2.60 &     1.63 \\
%LupoConfetti &   3.51 &   1.30 &   0.74 &   4.91 &   3.18 &   2.26 &     5.71 &     3.80 &     2.72 \\
%CandleSmoke &   3.64 &   1.04 &   0.49 &   1.82 &   0.63 &   0.29 &     2.62 &     0.84 &     0.39 \\
%WaterfallPan &   4.82 &   3.52 &   2.35 &   4.16 &   2.14 &   1.05 &     5.89 &     3.18 &     1.62 \\
%FountainLady &   3.21 &   2.01 &   1.31 &   3.24 &   1.87 &   1.10 &     4.08 &     2.49 &     1.47 \\
%\midrule
%ParkDancers &   5.41 &   4.27 &   3.05 &   2.29 &   1.00 &   0.63 &     3.91 &     1.50 &     0.87 \\
%StudioDancer &   3.70 &   1.11 &   0.61 &   3.29 &   1.70 &   1.01 &     4.24 &     2.25 &     1.32 \\
%\midrule
%\textbf{Total} &  49.29 &  26.51 &  17.01 &  33.81 &  16.55 &   9.61 &    49.35 &    23.26 &    13.34 \\
%\bottomrule
%\end{tabular}
%} 
%\end{table}
